Bias-Free Scalable Gaussian Processes via Randomized Truncations

Scalable Gaussian Process methods are computationally attractive, yet introduce modeling biases that require rigorous study. This paper analyzes two common techniques: early truncated conjugate gradients (CG) and random Fourier features (RFF). We find that both methods introduce a systematic bias on the learned hyperparameters: CG tends to underfit while RFF tends to overfit. We address these issues using randomized truncation estimators that eliminate bias in exchange for increased variance. In the case of RFF, we show that the bias-to-variance conversion is indeed a trade-off: the additional variance proves detrimental to optimization. However, in the case of CG, our unbiased learning procedure meaningfully outperforms its biased counterpart with minimal additional computation.

==> defs.tex <==
% COLORs
\usepackage[usenames,dvipsnames]{xcolor}
\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

% MARGIN + SPACING
%\usepackage[
%  letterpaper,
%  left    = 1.4in,
%  right   = 1.4in,
%  top     = 1.25in,
%  bottom  = 1.25in
%  ]{geometry}

%\author[2]{Author E\thanks{E.E@university.edu}}
%\usepackage[utf8]{inputenc}
%\usepackage[parfill]{parskip}
%\setlength{\parskip}{.5em}

% TEXT 
%\usepackage[final,expansion=alltext]{microtype}
%\usepackage[english]{babel}
%\usepackage{afterpage}
%\usepackage{framed}

% PARAGRAPH HEADER SPACING
\renewcommand{\paragraph}[1]{\textbf{#1}~}

% REFERENCE LINKS + COLORS
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{linkcolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}
%\usepackage{url}            % simple URL typesetting

% TABLES
\usepackage{booktabs}       % professional-quality tables
\usepackage{multirow}

% FIGURES
%\usepackage{graphicx}
%\usepackage[labelfont=bf]{caption}
%\usepackage[format=hang]{subcaption}
%
% LISTS
\usepackage{enumitem}

%% BIB + AUTHOR
%\usepackage{natbib}
%\usepackage{authblk}
%\usepackage{todonotes}
%\presetkeys{todonotes}{color=blue!30,size=\small}{}
%
%% MATH
\usepackage[makeroom]{cancel}
\usepackage{amsmath, amssymb}
\usepackage{amsfonts}       % blackboard math symbols
\usepackage[nice]{nicefrac}
%% \usepackage{comment}
%% \usepackage{siunitx}
%% \usepackage{dsfont}
%%\newcommand{\nf}[1]{\noindent{\textcolor{red}{\{{\bf Nick:} \em #1\}}}}
%
%% ALGORITHMS
%\usepackage[algoruled]{algorithm2e}
\usepackage[algo2e]{algorithm2e} 
%\usepackage{listings}
%\usepackage{fancyvrb}
%\fvset{fontsize=\normalsize}

% % tikz sutff 
\usepackage{tikz}
\newcommand\circled[1]{%
  \tikz[baseline=(X.base)] 
    \node (X) [draw, shape=circle, inner sep=0] {\strut #1};}
% \usetikzlibrary{fit,positioning,calc}
% \definecolor{light}{RGB}{220, 188, 188}
% \definecolor{mid}{RGB}{185, 124, 124}
% \definecolor{dark}{RGB}{143, 39, 39}
% \definecolor{highlight}{RGB}{0, 255, 0}
% \definecolor{gray10}{gray}{0.1}
% \definecolor{gray20}{gray}{0.2}
% \definecolor{gray30}{gray}{0.3}
% \definecolor{gray40}{gray}{0.4}
% \definecolor{gray60}{gray}{0.6}
% \definecolor{gray70}{gray}{0.7}
% \definecolor{gray80}{gray}{0.8}
% \definecolor{gray90}{gray}{0.9}
% \definecolor{gray95}{gray}{0.95}
% \definecolor{comment}{gray}{0.50}

% %\trivfloat{algorithm}
% %\renewcommand\algorithmname{ALGORITHM}
% \usepackage[utf8]{inputenc}
% \usepackage[english]{babel}
% \usepackage{amsthm}
% \newtheorem{lemma}{Lemma}


% \newcommand\dd{\mathrm{d}}

% \newcommand{\mcpoint}[2]{  
%   \fill[color=dark] (#1, #2) circle (7pt); 
%   \fill[color=light] (#1, #2) circle (5pt);
% }

% \newcommand{\LS}{\ensuremath { H^{-1} \! \left( E \right) } }
% \newcommand{\sLS}{\ensuremath { H^{-1} \left( E \right) } }
% \newcommand{\MLS}{\ensuremath { \widetilde{H}^{-1} \! \left( E \right) } }
% \newcommand{\sMLS}{\ensuremath { \widetilde{H}^{-1} \left( E \right) } }

% %\newcommand\T{\mathcal{T}}
% \newcommand\Keff{\widecheck{K}}
%\newcommand\Veff{\widecheck{V}}

% circled letter...
\newcommand{\tcirc}[1]{{\large \textcircled{\small #1}}}

%%%%%%%%%%%%%%%%%%%%%%
%%% math alphbbet %%%%
%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\blkdiag}{BlkDiag}
\newcommand{\given}{\,|\,}
\newcommand{\prox}{\textrm{prox}}

% bold lower
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bl}{\boldsymbol{l}}
\newcommand{\bm}{\boldsymbol{m}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bo}{\boldsymbol{o}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}

% bold upper
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bN}{\boldsymbol{N}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}

% greek letters
\newcommand{\blambda}{{\boldsymbol{\lambda}}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\newcommand{\bnu}{{\boldsymbol{\nu}}}
\newcommand{\bomega}{{\boldsymbol{\omega}}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bsigma}{{\boldsymbol{\sigma}}}
\newcommand{\bkappa}{{\boldsymbol{\kappa}}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bLambda}{{\boldsymbol{\Lambda}}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}



==> misc.tex <==
    % \subsection{Preliminaries}
    % Assume our goal is to estimate a quantity $Y_H := \lim_{ n\rightarrow H} Y_n$ for $n \in \mathbb{N}_+$ and $H \in \mathbb{N}_+ \cup \{\infty\}$, where the cost of computing $Y_n$ is nondecreasing in $n$, such that at a certain $n$ it may even become infeasible.
    % Examples include loop-like quantities such as the number of time steps used to evolve a numerical integrator, or the number of optimization iterations to perform \citep{beatson2019efficient}.
    % Instead of computing all $H$ terms, we randomly choose a truncation index from a categorical distribution $J \in \{1, ..., H\} \sim P(J)$, and truncate the computation at $n=J$ with probability $P(J)$, while up-weighting the surviving terms to facilitate unbiasedness.
    
    % John von Neumann and Stanislaw Ulam first proposed to estimate a series by random truncation and re-weighting. Since, this method has been widely applied in science and engineering (for a review, see \citet{beatson2019efficient}, Section 2.2.). Of particular interest is recent work in probabilistic machine learning applying it to estimate log marginal probability for deep generative models \citep{luo2020sumo, chen2020residual}.
    
    define $\Delta_i = Y_{i} - Y_{i-1}$ where we can apply the randomized truncation to the log marginal likelihood objective $Y_i \propto \log \vert \hat{K}_{i}\vert + \by^{\top}\hat{K}_{i}\by$ or to each of the terms that comprise it $Y_i := \log \vert \hat{K}_{i}\vert$, or $Y_i := \by^{\top}\hat{K}_{i}\by$.
%% below improve our theorems on RFF.
\textbf{RFF biases the log-likelihood terms}.
  Although $\approxK_M$ is an unbiased estimator of $\trainK$, we remain with biased estimates for the two terms comprising our learning objective (\cref{eqn:log_lik}):
  %
  \begin{align*}
    \Evover{\mathbb{P}(\omega)}{\log \vert \approxK_M \vert} &\ne \log \vert \trainK \vert, \\
    \Evover{\mathbb{P}(\omega)}{\by^\top \approxK_M^{-1} \by} &\ne \by^\top \trainK^{-1} \by.
  \end{align*}
  %
 because (for inverse quadratic)
   %
    \begin{align*}
    \Evover{\mathbb{P}(\omega)}{\approxK^{-1}} & \leq \Evover{\mathbb{P}(\omega)}{\approxK}^{-1} = \trainK^{-1}
  \end{align*}
  %
%   have to write such inequality for log determinant. also have to link the inequality to the fact we're overestimating the inverse quadratic.

These biases have clear implications for the hyperparameters. Underestimating $\logdet$ implies that, given a fixed set of parameters $\btheta$, when employing RFF, our model pretends to be simpler than it is. Equivalently, the complexity penalty is lessened.
After training in this manner, our model should be more complex compared to a GP trained with exact inference, and will have a larger $\logdet$. This could manifest when setting the lengthscale parameter $l^2$ to smaller values: For $l^2 \rightarrow 0$, we obtain a diagonal kernel matrix, i.e., $[\bK_{\bX\bX}]_{ij}=o^2 \; \text{when}\; i = j$ and zero otherwise. Another way to achieve high $\logdet$ is by setting higher observation noise $\sigma^2$, resulting in a kernel matrix with a large diagonal component.

% \begin{align*}
%     f(\bx) &\sim \GP{\mu(\bx)}{k(\bx, \bx')} \\
%     \intertext{\emph{GP regression} predicts the label $y$ as a latent GP plus Gaussian
%     observational noise: }
%     y &= f(\bx) + \epsilon, \quad \epsilon \sim \normaldist{0}{\sigma^2}
% \end{align*}
where $k(\bx, \bx')$ is called the
\emph{kernel} function defining the covariance between two training examples, and we
collect all pairwise kernel evaluations in an $n \times n$ matrix $\bK_{\bX\bX}$, i.e.,
$[K_{XX}]_{ij} = k(\bx_i, \bx_j)$. $\trainK$ is a kernel matrix with additional
homoskedastic Gaussian observational noise $\trainK= K_{XX} + \sigma^2 I$.
Typically $\mu(\bx)$ is set constant, and without loss of generality we will assume
$\mu(\bx)=0$. The kernel function $k(\bx, \bx')$ is often chosen to be the squared
exponential (a.k.a. RBF) kernel $k(\bx, \bx') = o^2\ex\mathbb{P}(\frac{-\vert \bx - \bx'
\vert}{2\mathcal{l}^2}) $or a Matérn kernel. This regression model has three
\emph{hyperparameters} $\btheta = \{o^2, \l^2, \sigma^2\}$ respectively the output scale
(controlling the magnitude of the GP signal) lengthscale (controlling the decay of the
correlation between neighboring datapoints) and observation noise (accounting for
unexplained variance).\\

Modern GPs are trained using stochastic optimization  \cite{gardner2018gpytorch}, often
in conjunction with neural network models, on GPUs.  Moreover, GP training is now
routinely accelerated using not only CG (\cref{sec:CG_background}) and RFF
(\cref{RFF_background}) but also inducing point methods and sparse variational methods
\citep{cutajar2016preconditioning, bauer2017understanding}.  The user has to specify a
fixed number of CG iterations, Fourier features, or inducing points to use, trading off
accuracy for speed.

% By reviving randomized truncation estimators from the 1950's that re guts of such approaches are ran
% Such approaches exchange the speed-bias tradeoff by a speed-variance tradeoff, introducing auxiliary variance into the model. The roots of such work come from work in the 1950's, forming unbiased estimates of infinate sums by randomly truncation and re-weighting.

% A significant body of work aims at reducing GPs' time
% complexity, either through approximating the exact GP model \citet{rahimi2008random}, or
% through reducing the exact GP computations to matrix vector multiplications (MVM)
% \citet{wang2019exact} which are easily parallelizable on a GPU.  One example of the
% former approach is Random Fourier Features (RFF) \citet{rahimi2008random}, which uses a
% randomized low-dimensional approximation to the kernel matrix, requiring $\bigo{J^3}$
% computation.
% passage that I wrote for the bias proofs. GP suggested to embed here
% Modern GPs are trained using stochastic optimization  \cite{gardner2018gpytorch}, often
% in conjunction with neural network models, on GPUs.  Moreover, GP training is now
% routinely accelerated using not only CG (\cref{sec:CG_background}) and RFF
% (\cref{RFF_background}) but also inducing point methods and sparse variational methods
% \citep{cutajar2016preconditioning, bauer2017understanding}.  The user has to specify a
% fixed number of CG iterations, Fourier features, or inducing points to use, trading off
% accuracy for speed. Because fast GPs rely on stochastic optimization, which is vulnerable
% to bias in the optimization objective \cref{eqn:log_lik} or its gradient in
% \cref{eqn:log_lik_deriv}, it is ever important to analyze and eliminate such biases
% \citep{tallec2017unbiasing, oktay2020randomized, chen2020residual, luo2020sumo,
% beatson2019efficient}.

\subsection{Algorithms}

If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
environments to format pseudocode. These require
the corresponding stylefiles, algorithm.sty and
algorithmic.sty, which are supplied with this package.
Algorithm~\ref{alg:example} shows an example.

\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

\subsection{Tables}

You may also want to include tables that summarize material. Like
figures, these should be centered, legible, and numbered consecutively.
However, place the title \emph{above} the table with at least
0.1~inches of space before the title and the same after it, as in
Table~\ref{sample-table}. The table title should be set in 9~point
type and centered unless it runs two or more lines, in which case it
should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{itemize}
    \item Unbiasedness - We show that fast GP methods like RFF and CG, when truncated
      early, result in biased estimates of the GP objective.
    \item When training models in this manner, we find that the resulting hyperparameters
      are biased w.r.t. their true value and the value obtained by training with Cholesky
      decomposition.
    \item By viewing both CG and RFF as a truncated series, we replace the deterministic
      truncation by a randomized one. Specifically, we deploy Randomized Telescope
      estimators which allow us to truncate early and still maintain unbiasedness.
    \item We show that de-biasing the loss function results in better predictions on test
      data, and higher-fidelity hyperparameters. Our method allows us to use very small
      numbers of CG iterations or RFF features, and maintain predictive performance that
      is equivalent to the Cholesky decomposition.
    \item Moreover, in large datasets where the Cholesky decomposition is infeasible, our
      method outperforms other scalable alternatives.
\end{itemize}


quantifying the bias that both CG and RFF introduce to the log marginal likelihood objective
GP training is sped up with fewer CG iterations or fewer Fourier features. Here, we test the hypothesis that early truncation of CG and RFF comes at a price of biased hyperparameters.
We generated synthetic data by sampling from the prior of a GP regression model with fixed hyperparameters:
\begin{align*}
    f(\bx) &\sim \GP{m(\bx)}{k({\mathbf{x}, \mathbf{x'}})} \\
    \by &= f(\bx) + \epsilon \quad \text{where} \quad \epsilon \sim \normaldist{0}{\sigma^2}
\end{align*}
and where $m(\bx) = \mathbf{0}$ and $k({\mathbf{x}, \mathbf{x'}})$ is the RBF kernel, parametrized by a lengthscale outputscale hyperparameters. Together with the observation noise $\sigma^2$, the model has three parameters (maybe show that actual RBF formula with parameters). In this experiment, we sweep over possible lengthscale values $(0.1, 1)$ and take a 500-dimensional sample $\by$.

We then fit two models: an RFF model that approximates the covariance matrix using $K$ samples, and a CG model that computes $\trainK^{-1}\by$ using $K$ iterations. In all the models, the observational noise and outputscale were fixed to their true value, while the lengthscale was trained.
% Exact GP model that computes the marginal likelihood using the Cholesky decomposition

We first train the hyperparameters of an \emph{exact GP model} that uses the Cholesky decomposition to compute the objective at every training iteration. We used the Adam optimizer, with a learning rate schedule of \db{Insert}, for 500 iterations.
Fixing the exact GP's optimized hyperparameters, we compute $\logdet$ and $\invquad$ using (1) an exact GP, (2) RFF and (3) CG. We varied the number of Fourier features between \db{insert X and X} and the number of CG iterations between \db{insert X and X}.


% In the left panel, we see that the exact training loss is qualitatively similar to the approximate one. The loss has less variance since we do not compute it using \emph{random} Fourier features. Here too, SS-RFF is slow to converge yet eventually outperforms RFF. To summarize, for RFF, it may be preferable to optimize the exact objective using $\bigo{N^3}$ operations rather than using a slow-to-train unbiased truncation.
% This experiment address s two questions \gp{the next two sentences don't ask questions \ldots}. First, we compare the training loss between biased, unbiased and exact methods \gp{what is it about the training loss that we care about? it's value? it's convergence?}. Second, we have shown in \cref{sec:bias} that the approximate loss optimized by CG and RFF is different from the exact Cholesky loss \gp{ what is the approximate loss? This has not been defined yet.}. Therefore here we log these two quantities at each training iteration and compare them. We again use the PoleTele dataset. \gp{Don't we use elevators?} \cite{asuncion2007uci}.


\paragraph{RFF and SS-RFF}
In the right panel of \cref{fig:loss_evolution_rff} we glean that RFF converges to an impoverished loss value, albeit improving as $J$ increases as predicted by the bias decay rate. SS-RFF ($\mathbb{E}[J]=700$) is unbiased and converges to a loss equivalent to Cholesky. Crucially, however, the convergence of SS-RFF is an order of magnitude slower. We attribute the slow convergence to the especially large truncation variance needed to counteract the slow $\bigo{1/J}$ decay of the RFF bias (see \cref{RFF_bias_theorem}).
In the left panel, we see that the exact training loss is qualitatively similar to the approximate one. The loss has less variance since we do not compute it using \emph{random} Fourier features. Here too, SS-RFF is slow to converge yet eventually outperforms RFF. To summarize, for RFF, it may be preferable to optimize the exact objective using $\bigo{N^3}$ operations rather than using a slow-to-train unbiased truncation.

\paragraph{CG and RR-CG}
In the right panel of \cref{fig:loss_evolution_cg}, we see that RR-CG converges as quickly and as accurately as an exact model, whereas CG converges to an inferior loss value. Here too, CG's bias decreases with $J$. RR-CG ($\mathbb{E}[J]=20$ \db{verify Luhuan?}) exhibits more variance than CG, yet it is only moderate and inconsequential due to the fast decay of CG's bias.
The exact loss in the left panel of \cref{fig:loss_evolution_cg} illustrates again that RR-CG and Cholesky are comparable in performance and running time. Interestingly however, as CG succesfuly optimizes its biased training objective, it fails to optimize the exact one. In fact, these two are inversly correlated: better values of the approximate CG objective lead to worse values in the exact objective.
We conclude that early-truncated CG successfully optimizes a distorted loss landscape. However, at least in this experiment, the exact loss landscape is quite different, leading to poor performance.

% However, with the aid of modern stochastic optimization techniques, such as Adagrad \citep{JMLR:v12:duchi11a} and Adam \citep{kingma2017adam}, these low-bias high-variance methods have seen empirical successes. 
%through techniques like unbiased randomized truncation \cite{kahn1955use}.
%\jpc{vague... a little bit more please}. \db{added in response:} 
%Briefly, this method applies to any biased term that can be written as a summation. Instead of computing the summation in full, this method randomly truncates the computation and up-weights the surviving terms to maintain unbiasedness. Thus, the bias is traded for an auxiliary truncation variance. 
% \db{The below paragraph describes stochastic gradients in general, not biasing and de-biasing, and not unbiased randomized truncation which I believe should be introduced}
% The key idea behind these algorithms is, instead of aiming for the exact gradient which is expensive or even intractable to evaluate, compute a cheaper, noisy but unbiased gradient estimate. 
% Given the same computational budget of biased counterparts, these randomized methods eliminate the biases but also introduces auxiliary variances.

%The success of these approaches builds upon general trends and developments in machine learning that favor first-order stochastic optimization \citep[e.g.][]{bottou2010large,JMLR:v12:duchi11a,kingma2017adam}
%and its potential regularizing effects \gp{cite}. 
%\jpc{i don't think this sentence is needed; it's kind of editorial, not strictly relevant.}

% One important bias reduction technique is \emph{unbiased randomized truncation} \citep{kahn1955use}, which applies to any biased term that can be written as a summation. Briefly, instead of computing the summation in full, this method randomly truncates the computation and re-weights the surviving terms to obtain an unbiased estimator.

% The technique can be applied to any biased term that can be re-expressed as a (potentially infinite) summation. Instead of computing the summation in full, unbiased estimates thereof can be obtained by randomly truncating the computation while up-weighting the surviving terms. However, such debiasing is not free: the random truncation adds variance into the procedure, which, when high, may be deleterious for optimization.

% Here, we theoretically investigate the biases introduced by CG and RFF to the GP log marginal likelihood objective and assess their practical ramifications on hyperparameter learning. Furthermore, we construct bias-free variants of CG and RFF for GP inference by randomly truncating the number of iterations/features and up-weighting intermediate solutions to maintain unbiasedness. Our bias-free methods converge to the (local) optimum equivalently to the Cholesky method
% To develop a better understanding for the outcomes of such GP approximations, we develop a theoretical analysis into their biased objectives. Moreover, we construct the bias-free variants of CG and RFF for GP inference by randomly truncating the number of CG iterations and the number of RFF features,   enabling the convergence to (local) optimum with stochastic gradient descent. 
%In this work, we investigate the biases arose from the common practice of early truncated CG and RFF, and then propose their bias-free variants with randomized truncation. 
%In this work, we introduce bias-free variants of two popular scalable GP methods---Random Fourier Features (RFF) \citep{rahimi2008random} and Conjugate Gradients (CG) \citep[e.g.][]{cunningham2008fast}.
% ---which makes these methods especially amenable to unbiased randomized truncation.
%In particular, we aim to quantify and remove the biases associated with CG and RFF hyperparameter learning. \jpc{redundant}
% When computing predictive distributions, the most expensive computations can be cached and amortized across all test points \cite{williams2006gaussian,pleiss2018constant}.
%Unlike other scalable GP approaches, the speed-accuracy tradeoff of these two methods is dynamically controllable. 
%The number of CG iterations and the number of RFF features can vary over the course of hyperparameter learning and prediction to elicit different levels of exactness. \jpc{what does "different levels of exactness" mean?  better approximation?  just say that}
%This property makes these two methods particularly well-suited to de-biasing via randomized truncation. \jpc{but i haven't been told what randomized truncation is, so I can't evaaluate this claim}
% This dynamic nature allows us to effectively negate predictive distribution bias simply by increasing the number of iterations/features for the cached computations.
% Consequently, bias mitigation is most crucial during hyperparameter optimization, where repeated computation of the marginal likelihood necessitates fast approximations.
% Biased hyperparameters may not be well suited to the observed data and may affect the quality of GP predictions.

% % Approximate methods unlock the use of GPs for large and previously unworkable datasets. Such computational shortcuts incur a speed-bias tradeoff which the field has just begun to scrutinize \citep{bauer2017understanding,burt2019rates}.
% We have analyzed the biases that both CG and RFF introduce to the GP's optimization objective.
% % We target the objective since it must be computed afresh throughout training, making methods like CG and RFF all but an imperative.
% % We establish that these two methods introduce biases that translate into two very different learned models.
% CG will tend to underfit, avoiding complex kernels at the price of compromised training errors.
% RFF will do the opposite, favoring an over-complicated model that fits the training data well.
% % In our experimental comparisons with exact GP training, we confirm that the biases in the objective translate into consistent biases in the recovered hyperparameters.
% % To eliminate these biases, Note that eliminating these biases simply by adding more Fourier features or CG iterations, will defeat the purpose of resorting to approximations in the first-place.
% % We cancel these bias by unbiased randomized truncation.
% Through randomized truncation, we convert the speed-bias tradeoff into a speed-variance tradeoff, which allows for unbiased optimization of GP hyperparameters.
% We find that training with debiased objectives overall converge to true optima.
% To this end, we view both CG and RFF as potentially infinite sums over iterations or Fourier features, which are in practice deterministically truncated. We then replace the deterministic truncation by a randomized one, enjoying the computational savings while maintaining unbiasedness \citep{kahn1955use, beatson2019efficient}.

% luhuan's version
\begin{proof}
\begin{align*}
\mathbb{E} \left[ \bar{\psi}_J \right] &= \mathbb{E} \left[ \sum_{j=1}^J  \frac{\Delta_j}{\mathbb{P} (\mathcal{J} \geq j )}\right] \\
&= \sum_{J=1}^H \left[ \left(\sum_{j=1}^J \frac{\Delta_j}{\mathbb{P} (\mathcal{J} \geq j)}  \right) \mathbb{P} (\mathcal{J}=J) \right], 
\end{align*}
exchanging the summation order, 
\begin{align*}
&= \sum_{j=1}^H \frac{\Delta_j}{\mathbb{P} (\mathcal{J} \geq j)} \left[\sum_{J=j}^H \mathbb{P} (\mathcal{J} = J) \right] \\
&= \sum_{j=1}^H \frac{\Delta_j}{ \mathbb{P} (\mathcal{J} \geq j )}  \mathbb{P} (\mathcal{J} \geq j ) \\
%&= \sum_{j=1}^H \Delta_j \\
&= \psi
\end{align*}

\subsection{Unbiasedness of the SS Estimator}
\label{appendix:SS_unbiased}
The SS estimator of \cref{eqn:ss_estimator} is unbiased, i.e., $\mathbb{E} \left[ \bar{\psi}_J \right] = \psi$.
\begin{proof}
\begin{align*}
\mathbb{E} \left[ \bar{\psi}_J \right] &= \mathbb{E}_J \left[ \sum_{j=1}^H  \frac{\Delta_j}{\mathbb{P} (\mathcal{J} = j )} 
\cdot \mathbbm{1}_{j=J} \right] \\
&= \sum_{j=1}^H  \frac{\Delta_j}{\mathbb{P} (\mathcal{J} = j )} \mathbb{E}_J[\mathbbm{1}_{j=J}]\\
&= \sum_{j=1}^H  \frac{\Delta_j}{\mathbb{P} (\mathcal{J} = j )} \sum_{J=1}^H \mathbb{P}(\mathcal{J}=J)\cdot \mathbbm{1}_{J=j}\\
&= \sum_{j=1}^H  \frac{\Delta_j}{\mathbb{P} (\mathcal{J} = j )} \mathbb{P} (\mathcal{J} = j )
=  \psi
\end{align*}
\end{proof}

\end{proof}

==> tables/table-ard-smalldatasets.tex <==
% RMSE and NLL
\begin{tabular}{lrrrrrrrrrrr}
\toprule
{}              & \multicolumn{3}{c}{\textbf{RMSE}}  && \multicolumn{3}{c}{\textbf{NLL}}  \\
 \cline{2-6}\cline{8-12}
Dataset         & \textbf{CG }                   & \textbf{RRCG}                 & \textbf{Cholesky}          
                && \textbf{CG }                  & \textbf{RRCG}                 & \textbf{Cholesky}            \\
\midrule
PoleTele        &  $-0.354 \pm -0.007$           &  $-0.458 \pm 0.010$           & $\mathbf{-0.464} \pm 0.006$  
                && $0.119 \pm 0.002$             &  $\mathbf{0.112} \pm 0.002$   & $\mathbf{0.112} \pm 0.002$      \\
Elevators       &  $0.429 \pm 0.012$             &  $\mathbf{0.425 \pm 0.013}$   & $\mathbf{0.425} \pm 0.013$    
                && $\mathbf{0.360} \pm 0.006$    &  $\mathbf{0.360} \pm 0.006$   & $\mathbf{0.360} \pm 0.006$     \\
Bike            &  $-0.971 \pm 0.008$            &  $-0.982 \pm 0.018$           & $-0.984 \pm 0.018$           
                && $0.040 \pm 0.005$             &  $\mathbf{0.035} \pm 0.002$   & $\mathbf{0.035} \pm 0.003$      \\
\bottomrule
\end{tabular}

